BitextEdit: Automatic Bitext Editing for Improved Low-Resource Machine Translation

Mined bitexts can contain imperfect translations that yield unreliable training signals for Neural Machine Translation (NMT). While filtering such pairs out is known to improve final model quality, we argue that it is suboptimal in low-resource conditions where even mined data can be limited. In our work, we propose instead, to refine the mined bitexts via automatic editing: given a sentence in a language xf, and a possibly imperfect translation of it xe, our model generates a revised version xf' or xe' that yields a more equivalent translation pair (i.e., <xf, xe'> or <xf', xe>). We use a simple editing strategy by (1) mining potentially imperfect translations for each sentence in a given bitext, (2) learning a model to reconstruct the original translations and translate, in a multi-task fashion. Experiments demonstrate that our approach successfully improves the quality of CCMatrix mined bitext for 5 low-resource language-pairs and 10 translation directions by up to ~ 8 BLEU points, in most cases improving upon a competitive back-translation baseline.

==> tmp.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\subsection{Pushing bitext refinement to the limit \eb{\textbf{QUESTION:} Need better title?}}
%
\begin{figure}[!t]
    \centering
    \includegraphics[width=5.2cm]{figs/cross-check.png}
    \caption{Translation quality of \textsc{en}$\rightarrow$\textsc{el} \textsc{nmt} models trained on $100$K samples~$\sim$~PoolA and $100$K~samples~$\sim$~x. x-axis indicates the \textsc{bleu} score of \textsc{nmt} models trained solely on PoolA that is also used to seed the mining of training data for bitext refinement (i.e., $r(.)$).\mg{I don't understand the figure }}
    \label{fig:cross_check}
\end{figure}
%
% Experiment Description
\mg{Let's talk about this section, I didn't get it.} The performance of bitext refinement models depends on the underline quality of the PoolA data we assume access to. 
As a result, we are interested in understanding how an improvement in the quality of PoolA interacts with the quality of the refined bitexts. Figure~\ref{fig:cross_check} presents translation quality results (i.e., y-axis) of \textsc{en}$\rightarrow$\textsc{el} models trained on the same amounts of data revised by bitext refinement models of varying quality. In principle, we can assume that a PoolA sample that yields \textsc{nmt} models of higher quality (i.e., here, higher \textsc{bleu}), results, subsequently, in training better bitext refinement models (i.e., x-axis). 
The trend presented in Figure~\ref{fig:cross_check} confirms our hypothesis: better refinement models generate revised bitexts that yield more useful training signal for \textsc{nmt} models, leading to an increase in \textsc{bleu}. At the same time, this observation further supports our previous claim that in  high-resource settings (i.e., PoolA with \textsc{bleu}~$>30$) our refinement models improve bitext quality even though this is not depicted in \textsc{bleu} for models trained on tens of millions training samples. Furthermore, the horizontal trendlines of Figure~\ref{fig:cross_check} put the observed improvements in perspective: first, regardless of the quality of PoolA the edits made by any of our bitext refinement models improve upon the original CCMatrix data (i.e., bottom line x$=$PoolB); second, all of the revised bitexts yield models that underperform an \textsc{nmt} trained on equal size of PoolA data (i.e., upper line x$=$PoolA). Treating the latter as an upper bound, we take this as an indicator that our models are still not perfect while further improvements in bitext editing can help yield further improvements in translation quality too. \eb{\textbf{IDEA:} Can we do an error analysis to give insights as to what are some of the issues?}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\iffalse
\begin{table*}[]
    \centering
    \begin{tabular}{lccccc}
    Method & \textsc{en$\rightarrow$oc} & \textsc{it$\rightarrow$oc} & \textsc{en$\rightarrow$be}  & \textsc{en$\rightarrow$mr} & \textsc{en$\rightarrow$sw} \\
    \textsc{cc}matrix &     $20.5$      &   $11.5$  &   $11.0$  &   $12.2$  &   $38.1$  \\
    Filtering         &     $18.1$      &   $11.7$  &   $9.8$   &   $12.2$  &   $37.6$  \\
    Back-Translation  &     $23.0$      &   $17.0$  &   $12.1$  &   $15.4$  &   $\mathbf{38.8}$  \\
    Bitext Refinement &     $\mathbf{26.0}$      &   $\mathbf{19.9}$  &   $\mathbf{13.0}$  &   $15.3$  &   $\mathbf{38.6}$  \\
    
    \addlinespace[0.2cm]
    
    & \textsc{oc$\rightarrow$en} & \textsc{oc$\rightarrow$it} & \textsc{be$\rightarrow$en}  & \textsc{mr$\rightarrow$en} & \textsc{sw$\rightarrow$en} \\
    \textsc{cc}matrix &     $24.3$  &   $11.6$  &   $9.8$   &   $13.0$ & $34.8$ \\
    Filtering         &     $17.8$  &   $11.1$  &   $7.8$   &   $11.3$ & $34.8$       \\
    Back-Translation  &     $27.7$  &   $15.6$  &   $9.6$   &   $15.1$ & $\mathbf{36.8}$ \\
    Bitext Refinement &     $\mathbf{28.7}$  &   $\mathbf{18.3}$  &   $\mathbf{10.8}$  &   $\mathbf{16.7}$ & $36.2$ \\
    \end{tabular}
    \caption{Main results}
    \label{tab:to_low_resource_main}
\end{table*}


\begin{table*}[!ht]
    \centering
    \scalebox{0.9}{
    \begin{tabular}{lrrrrrrrrrr}
    \toprule
     & \enoc & & \itoc & & \enbe  & & \enmr & & \ensw&\\
     \cmidrule(lr){2-11}
    \textsc{cc}matrix & $20.5$ &            & $11.5$  &             &  $11.0$       &    & $12.2$ &  & $38.1$ &  \\
    Back-Translation  & $20.8$ & \p $+0.3$  & $17.0$  & \p $+5.5$   &  $12.3$ & \p  $+1.3$ & $15.5$ & \p $+3.2$  & $37.6$ & \n $-0.5$    \\
    Bitext Refinement & $25.4$ & \p $+4.9$ & $19.8$ & \p $+8.3$ & $12.8$ & \p $+1.7$  & $15.8$ & \p $+3.6$ & $37.8$ & \n $-0.3$\\
    
    \addlinespace[0.4cm]
    
    & \ocen & & \ocit & & \been &  &\mren & & \swen & \\
    \cmidrule(lr){2-11}
    \textsc{cc}matrix &     $24.3$       &         &  $11.6$          &          & $9.8$    &            & $13.0$ & & $34.8$ & \\
    Back-Translation  & $26.6$ & \p $+2.3$  & $17.3$ & \p $+5.7$ & $9.9$  & \p $+0.1$ & $13.6$ & \p $+0.6$ & $33.8$ & \n $-1.0$ \\
    Bitext Refinement & $28.2$ & \p $+3.9$ & $18.5$  & \p $+6.9$ & $10.7$ & \p $+0.9$ & $16.4$ & \p $+3.4$ & $35.8$ &  \p $+1.1$\\
    \toprule
    \end{tabular}}
    \caption{Main results (all)}
    \label{tab:main_results_all}
\end{table*}
\fi
